Finite/fixed-time Stabilization of Linear Systems with States Quantization

This paper develops a homogeneity-based approach to finite/fixed-time stabilization of linear time-invariant (LTI) system with quantized measurements. A sufficient condition for finite/fixed-time stabilization of multi-input LTI system under states quantization is derived. It is shown that a homogeneous quantized state feedback with logarithmic quantizer can guarantee finite/fixed-time stability of the closed-loop system provided that the quantization is sufficiently dense. Theoretical results are supported with numerical simulations.

==> validation_simulation.tex <==
In this setcion, we consider a linear system with a emulated homogeneous stabilization controller \eqref{eq:q_sys}, where
\begin{equation*}
	A = \left[\begin{smallmatrix}
		1.5 & 3 \\
		0 & 1
	\end{smallmatrix}\right],\ B = \left[\begin{smallmatrix}
	1\\1
\end{smallmatrix}\right].
\end{equation*}
The control parameters is obtained by solving the LMIs \eqref{eq:LMI0} in Theorem \eqref{thm:hom_linear}, and $\mu=-0.2$, $\rho = 1$, 
\begin{equation*}
	G_\dn \!=\! \left[\begin{smallmatrix}
	1.1143 &  -0.1143\\
	-0.0857 & 1.0857
\end{smallmatrix}\right], P \!=\! \left[\begin{smallmatrix}
	1.6856 &  -0.1487\\
	-0.1487 &   0.6041
\end{smallmatrix}\right]
\end{equation*} 
\begin{equation*}
	S \!=\! \left[\begin{smallmatrix}
		1  & -1.33\\
		1  &  1
	\end{smallmatrix}\right], J \!=\! \left[\begin{smallmatrix}
		1 &  0\\
		0 &   1.2
	\end{smallmatrix}\right], \begin{aligned}
	K_0 &\!=\! \left[\begin{smallmatrix}
		-0.6429  & -1.8571
	\end{smallmatrix}\right],\\
K &\!=\! \left[\begin{smallmatrix}
	-2.2327  &  0.0327
\end{smallmatrix}\right].
\end{aligned}
\end{equation*}

In the simulation, we consider the quantization of states using both a uniform quantizer and a logarithmic quantizer. According to the Theorem \ref{thm:hom_lin_stab}, and Corallaries \ref{cor:1}, \ref{cor:2}, the uniform quantizer parameter $\Delta$ is set to 0.8, while the logarithmic quantizer parameter $c$ is set to 0.8676. The simulation results are presented in Figures \ref{fig:2} and \ref{fig:3}.

Figure \ref{fig:2} illustrates that the  homogeneous controller employing uniformly quantized states, achieves practical stability. In contrast, the homogeneous controller utilizing logarithmically quantized states demonstrates finite-time stability.
Figure \ref{fig:3} also provides insights into the behavior of the quantized states. With the uniform quantizer, the step size remains fixed, and the quantized states converge to a neighborhood of the origin. On the other hand, the logarithmic quantizer exhibits a decreasing step size as the states approach zero, ultimately leading to the convergence of all quantized states to zero.
%Regarding the control signal, once it converges to a neighborhood of the origin, the logarithmic quantization produces a smoother control signal compared to the uniform quantizer.
Overall, the numerical simulation results validate the feasibility of achieving stability and non-asymptotic stability in the emulated homogeneous control using quantized states.
\begin{figure}
	\centering
	\includegraphics[width=0.8\columnwidth]{norm.eps}
	\caption{Logarithm of the norm of state.}
	\label{fig:2}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{q_u.eps}
	\caption{Quantized states (left) and the contrl signals using quantized states(right).}
	\label{fig:3}
\end{figure}

